Pushing Your Point of View: Behavioral Measures of Manipulation in Wikipedia

As a major source for information on virtually any topic, Wikipedia serves an important role in public dissemination and consumption of knowledge. As a result, it presents tremendous potential for people to promulgate their own points of view; such efforts may be more subtle than typical vandalism. In this paper, we introduce new behavioral metrics to quantify the level of controversy associated with a particular user: a Controversy Score (C-Score) based on the amount of attention the user focuses on controversial pages, and a Clustered Controversy Score (CC-Score) that also takes into account topical clustering. We show that both these measures are useful for identifying people who try to "push" their points of view, by showing that they are good predictors of which editors get blocked. The metrics can be used to triage potential POV pushers. We apply this idea to a dataset of users who requested promotion to administrator status and easily identify some editors who significantly changed their behavior upon becoming administrators. At the same time, such behavior is not rampant. Those who are promoted to administrator status tend to have more stable behavior than comparable groups of prolific editors. This suggests that the Adminship process works well, and that the Wikipedia community is not overwhelmed by users who become administrators to promote their own points of view.

==> evaluation_human_evaluation.tex <==
While the blocked users data set validates the controversy measure
which forms part of the CC-Score, it says very little about the
clustering portion. To explore this issue, we use human evaluations of
the edit history of administrators during the 180 days after they
became an administrator. Without knowing anything about the CC,
Controversy, or Clustering scores associated with the edit history,
reviewers decided which general category, if any, the edits were
in. Results for the top and bottom 100 administrators ranked by each
score are presented in Figure \ref{figure:human_eval}.
\begin{figure*}
  \begin{center}
    \includegraphics[width=0.9\textwidth]{cats}
  \end{center}
  \caption{Human evaluation of the general category of edits (if any)
    for administrators directly after their RfA. The 100 highest and
    100 lowest scoring administrators for each metric (x-axis labels)
    are shown; because of overlap, 428 administrators are represented
    in total.}
  \label{figure:human_eval}
\end{figure*}

It is immediately apparent from Figure \ref{figure:human_eval} that
administrators with very low Clustering Scores were most often
classified as not editing in a coherent general category. Conversely,
users with a high Clustering Score were much less likely to be
topically focused. This implies that our article similarity metric
corresponds with an intuitive notion of topical similarity.

There are some interesting differences in the topic areas of the 100
admins with the highest C-Scores and the 100 with the
highest CC-Scores. As expected, the C-Score picks up a
substantial chunk of editors with no particular focus, while the CC
score does not. These are probably admins who are doing their job of
``policing'' controversy across a broad spectrum of topics. Somewhat
more surprisingly, the C-Score picks up more politically
focused editors while the CC-Score picks up many more who focus on
media and entertainment.

% The C-Score alone does not effectively discriminate between
% focused and unfocused editors in general, but does find users who
% focus on religion and politics. Users with high CC-Scores are even
% less likely than those with high Clustering Scores to be topically
% unfocused, perhaps due to the dearth of religion-focused
% administrators with high Clustering Scores.

Users with a high CC-Score are often focused on topics related to
media and entertainment. This is surprising, given that neither the
Controversy nor Clustering Scores discriminate between users focused
on media and those who are not. The CC-Score multiplies page-level
controversy and clustering scores, effectively looking for articles
which are both similar to other articles that the user has edited and
are controversial. Religion-focused editors edit very controversial
pages, but those pages are not particularly clustered according to our
metric. Conversely, geography-focused editors edit non-controversial
but clustered pages. Media-focused editors seem to strike a balance
between controversy and clustering which results in high CC-Scores.

The apparent lack of clustering for religion-focused editors may be
because articles related to religion stand out to human reviewers,
forming natural categories. A user who has edited a few articles
related to a specific religion might reasonably be classified as
focusing on religion, whereas editing a few articles related to places
does not signify a geography-focused editor. The CC-Score can be
interpreted as compensating for this effect by giving more weight to
clustered articles which are controversial.

